A Marker-based Neural Network System for Extracting Social Determinants of Health

Objective. The impact of social determinants of health (SDoH) on patients' healthcare quality and the disparity is well-known. Many SDoH items are not coded in structured forms in electronic health records. These items are often captured in free-text clinical notes, but there are limited methods for automatically extracting them. We explore a multi-stage pipeline involving named entity recognition (NER), relation classification (RC), and text classification methods to extract SDoH information from clinical notes automatically. Materials and Methods. The study uses the N2C2 Shared Task data, which was collected from two sources of clinical notes: MIMIC-III and University of Washington Harborview Medical Centers. It contains 4480 social history sections with full annotation for twelve SDoHs. In order to handle the issue of overlapping entities, we developed a novel marker-based NER model. We used it in a multi-stage pipeline to extract SDoH information from clinical notes. Results. Our marker-based system outperformed the state-of-the-art span-based models at handling overlapping entities based on the overall Micro-F1 score performance. It also achieved state-of-the-art performance compared to the shared task methods. Conclusion. The major finding of this study is that the multi-stage pipeline effectively extracts SDoH information from clinical notes. This approach can potentially improve the understanding and tracking of SDoHs in clinical settings. However, error propagation may be an issue, and further research is needed to improve the extraction of entities with complex semantic meanings and low-resource entities using external knowledge.

==> backup.tex <==
Introduction

% Firstly, Then, a relation classification model is introduced to match pairs of trigger-argument entities candidates predicted by the extractor. In the stage three phase, we train the text classification model to category labeled argument to subtypes, separately.

% What is health equity?
% user, community, society 

% Many factors influence health, which can be classified into five main categories known as health determinants: genetics, behavior, environmental and physical influences, medical treatment, and social factors. These five categories are linked. Social determinants of health include economic and social factors that affect health. These conditions are shaped by socioeconomic standing, which is people's money, power, and resources, which are influenced by socioeconomic and political forces (e.g., policies, culture, and societal values). Education, occupation, or income might affect a person's socioeconomic status. All of these elements affect people's health and the health of their communities.

% These additional elements are collectively referred to as social determinants of health (SDOH). Individual variables (including education, housing, and money) and neighborhood or community factors (like crime and poverty) are examples of SDOH that are generally regarded the root causes of medical disorders that require treatment (like access to healthy foods or community support services and neighborhood safety or walkability).

% Social determinants of health (SDOH) are the environmental conditions in which people are born, live, learn, work, play, worship, and age that influence a wide range of health, functioning, and quality of life outcomes and risks. SDOH is based on what the World Health Organization (WHO) defines as "the conditions in which people are born, grow, live, work, and age. SDOH are conditions in people's lives that affect the quality of life and health outcomes. While SDOH affects patient risk and clinical outcomes, this non-clinical information is often locked away in unstructured clinical notes. SDOH encompasses a wide range of conditions including, but not limited to, substance use, living conditions, employment, education, racism, geography, and pollution. SDOH may lead to a reduction in life expectancy, especially for specific populations~\parencite{blizinsky2018leveraging}. Knowing SDOH and the behaviors influenced by these social factors can inform clinical decisions and improve health outcomes~\parencite{daniel2018addressing}. The use of SDOH has the potential to improve diagnosis, treatment planning, and patient outcomes in different populations~\parencite{braveman2014social}.

% However, SDOH also contributes to widespread health disparities and inequities. For example, people without access to healthy food in grocery stores are less likely to have good nutrition. This raises their risk of health conditions such as heart disease, diabetes, and obesity - and even reduces life expectancy relative to those with access to healthy foods. A physician who specializes in natural language processing technology demonstrates how it can assist clinicians in sorting through unstructured data to manage the chronic disease better and promote health equity~\parencite{thornton2016evaluating}. Social determinants of health typically fall into several categories: economic stability, food insecurity, social background, environment, education, and health care system. Natural language processing allows providers to unravel the social determinants of health, giving them a complete picture of each patient's situation. In addition to basic sentiment analysis, a sophisticated NLP platform is needed to extract key concepts and relationships, such as identifying social isolation issues, transportation issues, and cultural factors, which can be used to improve understanding and customer satisfaction~\parencite{marmot2009action}.

% The COVID-19 pandemic has further exacerbated health disparities, underscoring the importance of SDOH for better understanding how to address patient complexity and health equity via accessible telemedicine. Data collected during the pandemic indicates that interest and activity around SDOH remains high and points towards telehealth as one important and ongoing facilitator for SDOH efforts. At the outset of the pandemic, the volume of in-office primary care visits dropped precipitously across the United States and remained below prior levels through the end of 2020. In the absence of opportunities to engage with patients face-to-face, an increase in telehealth and virtual visits allowed providers to reach their patients (and vice versa) and maintain regular care. As in-office visits have returned closer to pre-pandemic levels, telehealth and virtual visit rates have slowed, but remain far above the levels seen at the start of 2020. In addition to clinical care, these shifts had a significant effect on SDOH screening and action. Across the OCHIN network of community health centers (CHCs), there was a substantial decline in overall SDOH screening activity captured in electronic health records (EHR) that corresponds with the drop in in-office visits starting in March of 2020. However, this was partially offset by a rapid increase in the proportion of SDOH screens being conducted in telehealth visits (Fig. 1) and, in both April and May of 2020, more SDOH screens were conducted via telemedicine (including virtual visits with video and those conducted by telephone only) than in all other encounter types combined. By October 2020, SDOH screening volumes were back up to pre-pandemic levels, but through mid-2021, telehealth visits have continued to account for roughly 15-20% of monthly SDOH screenings – up from effectively 0% at the start of 2020.

% A growing body of research highlights the importance of upstream factors that influence health and the need for policy interventions to address those factors—in addition to clinical approaches and interventions aimed at modifying behavior.

% Impact of the COVID-19 Pandemic on the Hospital and Outpatient Clinician Workforce
% reduce clinician documentation burden

% Electronic health records (EHRs) that document patient status and all elements of clinical care have the potential to considerably assist quality improvement and surveillance activities while also revolutionizing clinical research.

% A physician expert in natural language processing technology explains how it can help clinicians sift through unstructured data to better manage chronic conditions and boost health equity. NLP help clinicians identify at-risk patients, and how it can help clinicians and health IT leaders uncover insights into social determinants of health and advance population health efforts.

% many risk factors for disease, disease severity and disease progression are features that either cannot be coded or are rarely coded, because they do not impact medical insurance reimbursement through Medicare, Medicaid or private healthcare coverage. These signs, symptoms and social determinants of health are captured in medical records by clinicians, but rarely translate to what exists in the structured data.

% First, let's consider a case where risk factors are known for a disease. NLP can be configured to search the medical records for those known factors and determine which patients have these features present. For example, NLP can determine which words are diseases, procedures, signs or symptoms – known as "entity recognition" – and then the technology can link those entities to known ontologies or terminologies to build a rich feature set of potentially predictive features. These features then can be fed into other clustering or machine learning pipelines alongside standard structured data to determine potentially at-risk patients. This use of NLP to create features for machine learning is a powerful combination.

% for example, an elderly patient at admission: "This gentleman was brought in by ambulance having been found lying outside his home. He lives alone -> With NLP, this statement can be transformed into structured data that reads: "Social isolation; widowed; walks with assistive device; no transportation." Having this information in a structured format against not just one patient, but an entire population, means providers can better identify those patients at higher need and higher risk.

% SDoH can help with population health initiatives. Our understanding that the sickest in a population account for the majority of healthcare spending is not new. This is why the challenge has always been to identify and manage patients earlier, and when their respective disease is less severe, so they do not progress to more resource-intensive needs.

% With the increasing expansion of clinical data produced by health organizations, efficient information extraction from these free-text clinical notes will be advantageous for optimizing clinical ward operations and gaining a deeper understanding of the progression of patient care and disease. However, qualitative information about patients’ lifestyles is usually documented in unstructured clinical notes in EHRs. However, SDoH information is more frequently documented in unstructure clinical notes than structured data fields. These critical patient information is not accessible to computerized methods, which our ability to study these linkages is limited, and must first be translated into a structured form in order to support downstream secondary use applications. To address this issue, there is a growing push to develop techniques for automated SDoH extraction. When healthcare teams screen for and identify social risks, the information is typically recorded in free-text fields or unstructured data~\cite{hatef2019assessing}. 

% When clinical teams screen for and identify social risks, that information is more often documented within free-text fields, or unstructured data~\cite{hatef2019assessing}. The majority of health systems aim to incorporate SDoH data into the patient's health record. Nevertheless, they encounter several compatibility issues throughout the implementation phase. Recent studies aims to automate the incorporation of unstructured SDoH data into structured EHR data. Traditionally, this information has been manually extracted from unstructured data through medical record review, which can be time-consuming, especially during pandemic, and the extensive documentation burden can increase burnout, reduce job satisfaction, and lead to medical errors and adverse events. However, new improvements in natural language processing (NLP) enable more efficient, automated methods to extract and evaluate valuable data from existing EHRs data~\cite{conway2019moonstone}.

% Flat NER has been well studied and is usually viewed as a sequence labeling problem~\cite{lample2016neural}. However, nested entities also widely exist in real-world applications due to their multi-granularity semantic meaning (Alex et al., 2007; Yuan et al., 2020), which generally be solved by the multiple sequence labeling framework since tokens have multiple labels (Finkel and Manning, 2009) or span-based classification model. The rules or patterns may not be generalisable due to the specific writing style of individual clinicians. However, a machine learning approach is not fully advanced in clinical named entity recognition due to a lack of available training data

% Automatic Extraction of Social Determinants of Health from Clinical Notes
% NLP methods: language models and learning architectures (e.g., transformers), named entity recognition, relation extraction,  semantic role labeling
% NLP software tools: Any general or specific NLP tools for health data such as clinical notes, social media, biomedical literature etc. 
% NLP applications: Uses of NLP for clinical research or operation, examples including pharmacovigilance, clinical decision support, phenotyping, predictive modeling, risk prediction, social media mining etc.
% transformer-based architectures

% Various paradigms for nested NER have been proposed in recent years. One popular direction is the span-based approach that learns deep representation for every possible span and then classifies it to the corresponding type (Zheng et al.,2019; Xia et al., 2019; Wadden et al., 2019; Tan et al., 2020; Wang et al., 2020; Yu et al., 2020). By leveraging the large-scale pretrained language model, several works show that the simple model structure for span representation and classification can achieve satisfactory results (Luan et al., 2019; Zhong and Chen, 2021).





% Marker 
Figure 3 shows the overall framework of marker-based system. Formally, marker-based ner system takes the given prefixed label token and the text sequence (x) as input, and generates the linearized SEL (y) which contains the extracted information from x based on marker s:

y  = MODEL( s + x )

where x = [x1, x2, ... xn ] is the text sequence, s = [s1, s2, ..., sp] is the special marker token constructs a marker-based prompt and uses it as a prefix during training and prediction. and y  = [y1,y2,...,ym] is the sequence of prediction.

Specifically, corresponding to the event structure, the marker contains three types of token segments: 1) Trigger-Type: the targeted trigger type in the specific information extraction task, such as “drug“ in the NER task; 2) Argument-Type: the targeted argument type in the specific information extraction task, such as “type“ in the NER task; 3) Special tokens (<Trigger>, <Argument>) which are added before each Trigger-Type, Argument-Type, and input text sequence. All markers are concatenated and put before the original text sequences.


As shown in Figure 3, the entire input for marker-based ner model is the form of: 

s + x = [s1,s2,...,sp,x1,x2,...,xn] 

for example, if we prepend marker <Argument><Drug><StatusTime> [text] indicates extracting the StatueTime Argument for drug event from the sentence. Given the markers, ner model first encodes the text x, then predict the entities y specific to the senmatic meaning of the markers using an CRF architecture.

We found that the label-based/senmatic meaning prompt can: 1) effectively guide the sequential tagging model, so that ; 2) adaptively control which to predict, which to match so that semantic knowledge across different labels and tasks can be better shared. pass from trigger to the argument.

Given marker s and text x as input, marker-based ner model extract targeted information by sequential labeling.

Compared with previous IE studies which treat labels as specific symbols, the marker-based ner paradigm treats labels as natural language tokens with semantic meaning. 




\subsection{Discriminator/Relation Classification Model}

% Relation classification (RC) is a fundamental task in Natural Language Processing (NLP) that seeks to discover semantic relationships between pairs of marked entities in given sentences or documents (instances). Relation extraction (RE) is an essential information extraction task that aims to determine the relationships between entities in unstructured texts. Many researchers have recently focused their attention on document-level RE ~\parencite{sahu2019inter}, which aims to identify the relations of all entity pairs in a document since it is more in demand than sentence-level RE in various realistic scenarios.

% Generally, one document comprises numerous entities, and an entity may be mentioned multiple times in various phrases. Furthermore, a single entity may be involved in several legitimate connections, and different references to the same entity express different interactions. As a result, document-level RE is more difficult to master than sentence-level RE. Document-level relation extraction is more difficult than typical sentence-level connection extraction since one entity in a document may be cited numerous times and connected with multiple relations. On the other hand, most document-level relation extraction methods do not distinguish between mention-level and entity-level features and instead use a simple pooling operation to aggregate mention-level data into entity-level features. As a result, the varied semantics of an entity's several references are neglected. Existing document-level RE approaches collect mentions of an entity (mention-level features) to derive its representation (entity-level feature) first since relation categorization is done on the entity level. Finally, a fixed entity representation is provided in the relation classifier~\parencite{yao-etal-2019-docred}.

After the extractor has obtained the pair of entity candidate set C, the discriminator aims to 

In view of this, we propose a binary relation classification, which makes full use of both boundary and content of span. It first predicts the probability of pair of trigger entities and argument entities link or not. 

In the input sequence X, there may be multiple entities of a particular category. This means that multiple trigger and argument entities could be predicted. To match them, 

For any given span, we calculate the probability of pair of entity candidate: 

probability(trigger_i, argument_j | Sentence, Marker) = sigmoid( )

threshold.

\subsection{Pre-trained Word Representation}

% Text Encoding
% For text X = [x1, x2, ..., xN ] with N tokens, we first generate the contextual embedding xic with the pre-trained language model, xc 1, xc 2, ..., xc N = PLM(x1, x2, ..., xN ) Then, we concatenate xic with word embedding xiw, part-of-speech embedding xp i and character embedding xch i , and feed the concatenated embedding xi into a BiLSTM (Hochreiter and Schmidhuber, 1997) to obtain the token representations {hi}.

We explore three sets of embeddings: Flair, T5 and BERT. Social media texts are brief and informal. Drugs and chemicals are typically described in descriptive, nontechnical language with spelling errors. These issues challenge social media NER. Some medications, like ``all-trans-retinoic acid'', contain morphologically difficult parts. Yet, similar-structured phrases still generally represent similar things~\cite{zhang2021identifying}. Hence, the way we represent words (i.e., the embeddings we use) can have a direct impact on performance and bias. We describe each embedding we use in our study below:

% Character-level representation and Contextualized character-level embeddings
\paragraph{Flair~\cite{akbik2018coling}.} \Mycite{akbik2018coling} recently proposed a Flair contextual string embeddings (a character-level language model). Specifically, we use the embeddings in the HunFlair extension of the Flair package~\cite{weber2021hunflair}, which is pre-trained on a corpus of three million full-text articles from the Pubmed Central BioC text mining collection~\cite{comeau2019pmc} and about twenty-five million abstracts from PubMed. Unlike word embeddings mentioned above, Flair embeddings are a contextualized character-level representation. Flair embeddings are obtained from the hidden states of a bi-directional recurrent neural network (BiRNN). They are trained without any explicit notion of a word. Instead, Flair models a word as sequences of characters. Moreover, these embeddings are determined by the text surrounding them, i.e., the same word will have different embeddings depending on its contextual usage. The variant of the Flair embedding used in this study is the Pooled Flair embedding~\cite{akbik2018coling}. Furthermore, we use the forward and backward representations of Flair embeddings returned from the BiRNN. Intuitively, character-level embeddings can help improve model predictions with better OOV handling. 

% Classic word embeddings
\paragraph{T5-3B~\cite{pyysalo2013distributional}.}  In this paper, we use the Word2Vec embeddings pretrained on PubMed and PubMed Central (PMC). The embeddings are publicly released as part of the FLAIR package. It is important to state that word embeddings have a major limitation. Word embeddings use a distinct vector to represent each word and ignore the internal structure of words, which models are not particularly good at learning rare or out-of-vocabulary (OOV) words in the data. The growing number of emerging chemicals and drugs with their diverse morphological forms makes recognizing chemical entities on social media platforms particularly challenging. Another challenge posed by user-generated content is its unique characteristics and use of informal language, typically short context, noisy, sparse, and ambiguous content. Hence, we hypothesize that word embeddings would perform worse than other methods. However, it is unclear how these differences can impact bias.

% Embeddings from pretrained transformers (BERT, XLM, GPT, RoBERTa, XLNet, DistilBERT etc.)
\paragraph{BERT~\cite{devlin-etal-2019-bert}.} 
We also evaluate transformer-based embeddings. Specifically, we use the BERT variant ``bert-base-uncased'' available Flair and HuggingFace~\cite{wolf-etal-2020-transformers}. BERT was pre-trained using the BooksCorpus (800M words) and English Wikipedia (2,500M words)~\cite{devlin-etal-2019-bert}. Furthermore, BERT embeddings are based on subword tokenization, so BERT is able to handle OOV. Intuitively, it fits somewhere between Flair (generating word embeddings from character representations) and Word2Vec (which learns embeddings for each word independently). Likewise, each word representation is context-dependent. Hence, BERT is better at handling word polysemy by capturing word semantics in context. 


% SHAC is comprised of 4480 social history sections with detailed annotations for 12 critical SDOH. SHAC utilizes clinical notes from MIMIC-III [12] and an existing dataset from the University of Washington (UW) and Harborview Medical Centers. It includes event-based annotations for more than 55K annotated spans and 18K distinct events across four note types.

% This work utilized two clinical datasets without SDOH annotations: MIMIC-III and UW Dataset. MIMIC-III (referred to here as MIMIC) is a publicly available, deidentified health database for over 40K critical care patients at Beth Israel Deaconess Medical Center from 2001– 2012 [12]. MIMIC contains clinical notes, diagnosis codes, and other data. This work utilized 60K MIMIC discharge summaries. The UW Dataset is an existing clinical dataset from the UW and Harborview Medical Centers generated between 2008–2019. This work utilized 83K emergency department, 22K admit, 8K progress, and 5K discharge summary notes from UW Dataset. An existing corpus with SDOH an- notations created by Yetisgen and Vanderwende, YVnotes, was used for model training during active learning




% Error Analysis



==False Prediction== 

"No illicit drug use including IV drug use."

Our model predict ``illicit drug use'' and   ``IV drug use'' as the Drug trigger, but ground truth only has ``illicit drug use'' ignore the fact the IV drug included in illicit drug, and in semantic meaning they are mentioned the same thing.

Here we found an opposite example 

"Illicit drugs:  current marijuana use, cocaine quit 5 years ago"

In this case, the ground truth of Drug trigger is ``marijuana use'' and ``cocaine''. But our model predict ``Illicit drugs'' as the trigger. This example indicates that our model confused current vs past events in a sentence. They cannot identify two drug trigger in the same sentence with different temporal tenses. 

''Former heavy drinker, currently drinks three beers daily.''

"She drinks 2-3 alcoholic beverages per week."

Our model predict ``drinks'' as trigger, while ground truth is ``alcoholic''. Based on the criteria~\Mycite{}, the phrase describing general substance (i.e. alcohol, tobacco, or drug) or substance-related verb, such as drink both can be recognized as trigger. both could potentially be correct. One reason for the ground truth being alcoholic is that it is more specific. If there is more than one entity, the annotator may choose a more specific entity. But our model fails to understand the underlying semantic meaning. Thus, it incorrectly predicts the trigger with more general terms.  This is also very common for Tobacco trigger, for example, our model incorrectly predict ``smokes'' as trigger instead of ``cigarettes''.  and there is also similar in Employment event, for example, our model predict ``worked'' as trigger instead of ``retired''. 

==Missing Prediction==

==complex senmatic meaning==

''Currently at a rehab facility, but previously living with his wife at home.''  and "valium, alprazolam, and a small amount of vodka" 

The ground truth in this case for LivingStatus is ``a rehab facility'', but our model fail to predict LivingStatus. This error suggests that the our model is incapable of understanding complex senmatic meaning to undertand a rehab facility represent the residence. A future interesting research avenue would explore methods for incorporating external knowledge bases, similar to recent work on common sense generation~\cite{xing2021km}, into transformer models to address these errors. Similarity, In the second case, we fail to recognize the vodka as the alcohol type.

The ground truth is that the person lives in a rehab facility, but our model didn't predict it correctly. This shows that our model lacks the ability to understand the semantic meaning of a rehab facility as a residence. Future research could focus on incorporating external knowledge bases, like the recent work on common sense generation, into transformer models to fix these errors. Similarity, In the second case, our model failed to identify the alcohol type as vodka.

''Per OMR notes, she drinks a glass of wine a few times a week.''

For the quantitative related arguments, such as amount, frequency, and duriation, our model is easier predict part of entity, for example, in this case, the ground truth for amount argument is ''a glass of wine'', but our model predit ''a glass'' as amount and ''wine'' as type. 

In terms of quantitative arguments such as amount, frequency, and duration, our model is tend to predict part of an entity, for instance, in this case, the correct amount argument was "a glass of wine" but our model predicted "a glass" as the amount and "wine" as the type.

==discontinue entity==

"He has a history of polysubstance abuse: EtOH, heroin, IVDU, benzo"  

The goundtruth for Type argument of Drug trigger are "heroin", and "bento". ''IVDU'' is the method argument. our model consider "EtOH, heroin, IVDU, benzo" as a whole entity for type arguemnt.  This indicated that our model fail to extrct the discontinue entity. And our model continue incorrectly recognized IVDU as type argument instead of method.  

Similarity, for short sentence"pipe smoker", we misclassifier pipe as Type instead of Method. This indicated that Type and Method  argument are hard to differenciated if the sentence including less information are short. 

"No IVDU, cocaine use"

For this sentence, there are two drug trigger, ''IVDU'' and "cocaine", in one short sentence. Our model identify them as an entire entity "No IVDU, cocaine use", which indicate that our model incorrectly identifies IVDU and cocaine are two different drug event by ignoring Pre- and post-modifiers verb, adjective, and adverb  which will affect the sentnece sematic meaning. 

专有名词关于职业的无法识别 an architect

“Retired postal worker; formerly chief operating officer of post office”

our model identify the type argument as "Retired postal worker", but ground truth is "chief operating officer of post office". Which including more detail. 

==Fail to handle the Prepositions==

"Works in finance at Mass Eye & Ear. "

Our prediction is for type argument of Employment event is "finance" which is the part of ground truth "finance at Mass Eye & Ear" This indicated that our model fail to handel the longer phrases with prepositions. Similarity, we predict Type arguement for Employment as "insurance" instead of "in insurance"

The patient social history in Task B are more complex and having different writing style, For example, 

"Tobacco Use: \_   Alcohol Use: \_   Drug Use: \_"

Our model predict the Tobacco, Alcohol, and Drug trigger in this sentence. But  the ground-truth is there is no event due to "\_" means nothing happened, which unseen in the MIMIC-III data.  This example indicates that our model cannot undertand the senmetic meaning which unseen in the training dataset. Similar to the sentence "+methamphetamines +heroin +cocaine", our model predict this as whole drug entity, maybe because  the system believe it all belongs to drug. However, it neglected the fact that these three word metioned different drug usage. 

In the task B notes, the sentence are more complicated and longer than the mimic-III data, and havin Irregular spelling issue. For example, "unknown etoh use but has been documented as non-etoh using previously"  and "Nondrinker". We mis-predict the Alcohol argument as "etoh use" instead of ground-truth "non-etoh using", which including more information, represent the direction of alcohol usage. and We missed the prediction of "Nondrinker". This indicated our model cannot handle the adjective adverb which may affect the sematic meaning. 

''Alcohol Use: Currrently drinks 1 drink/night on the three days/week that he works. On all other nights he goes out with friends and has 3-4 drinks per night. (Total of 15-19 drinks/week). He has had 5 or more drinks in one sitting a few times over the last year, less than 1x/month. There was ~ a 1 year period of time 13 years ago when he went out a lot more so drank much more. Due to being told during this hospitalization that he has a problem with his liver, he volunteered that he would like to quit drinking. No hx of EtOH w/d or seizure per ED provider note. ''

And in task B, there is a lot Long and difficult sentences, such as the above example, which we incorrectly predict "EtOH"  and "drinking" as Alcohol trigger. This indicated our model confused future and none. 

"Heavy drinking for 2-3 years following her divorce which was 3-4 drinks a night. Since then continued drinking for several years."

The patients in the Task B have more complex social history. Therefore, The clinical note records more information. Some of them are may discribe the same event and annotator just label the event with more information. For example, in this case, the ground-truth of Alcohol trigger is "EtOH" at the front of sentence. and the second and third sentence are mentioned the same thing as the first one. So in this case, annotator didn't consider them as independet event. But our model fail to recognize this. Hence, we also predict "continued drinking" and "alcohol" as trigger. 

Some sentence in the task B are very short 

Task B have more noun  about the type arguement of employment, like Going to school, 

"Grandmother alive ('in her 90s'), was previously living with her but feels she is too unwell to deal with him at the house" and "Daughter works at Snoqualmie Valley Hospital Pt states that his son **lives** in [LOCATION] at the moment."

There are two sentence about the LivingStatus. The first one we missed prediction about the trigger "living", because our model fail to understand the grandmother is lived with patient, which would be consider the relavent LiviningStatus by annotator.  And the second sentence we incorrectly predict the trigger "lives", which negelect that the fact they are lived independent, which event would not be including in the patient livingstatus event. 

For the sentence, "History of incarceration.", we missed the trigger prediction, Because our model fail to understand the  "incarceration" represent the place for living. 

long document may have more error 

What's more, our relation classification model perform worse for the long documents in task B. 

For the sentence: "EtOH up to 8 beers a night, a few times per week Denies IVDU", we incorrectly predict the frequency argument as "a night", but the ground-truth is "a night, a few times per week" which contain more information. 

For the sentence, "Denies alcohol or illicits since last discharge", we incorrectly predict the subtype of StatusTime for alcohol as none. One of the possible reason is our ignoring the meaning of "last discharge" which represent the past status. (Ground-truth is past). 

In the task B, there is a lot of spoken writing style, which make even hard for our model to recognize the entity 

And For the Task A, If we trian the model with in-domain data, most of error casued by wrting style and wording can be fixed. But the adjectives, verb, and adverbs close to interesed entity with specific sematntic meaning still cause lot of issue to extract the correctly entities.  

% - patients with high risk social determinants of health are more likely to be misrepresented by extraction models 
% - patients with more severe social needs will have more complex social and behavioral histories. These more complex histories are harder to annotate, and I'll argue that they're also harder to extract. some of the patients especially well for some of the patients that have very, very complex social and behavioral histories
% - this drug history is just an example of social and behavioral history. There's a **verb** that that gives you the status label. 
% - And certainly these are **the types of cases** that led to **the lower performance in Task B**, where the where the models were being applied to these actively selected notes, where the **active selection mechanism** was kind of inherently searching out for these difficult to classify examples.
% - MIMIC simple cases UW more complecated 
% - **be more likely to be misrepresented by the use of these types of extraction systems.** 
% - ==high level thoughts: special attention needs to be paid to these less frequent but more complex cases== 


